Solving Min-Max Optimization with Hidden Structure via Gradient Descent Ascent

Many recent AI architectures are inspired by zero-sum games, however, the behavior of their dynamics is still not well understood. Inspired by this, we study standard gradient descent ascent (GDA) dynamics in a specific class of non-convex non-concave zero-sum games, that we call hidden zero-sum games. In this class, players control the inputs of smooth but possibly non-linear functions whose outputs are being applied as inputs to a convex-concave game. Unlike general zero-sum games, these games have a well-defined notion of solution; outcomes that implement the von-Neumann equilibrium of the "hidden" convex-concave game. We prove that if the hidden game is strictly convex-concave then vanilla GDA converges not merely to local Nash, but typically to the von-Neumann solution. If the game lacks strict convexity properties, GDA may fail to converge to any equilibrium, however, by applying standard regularization techniques we can prove convergence to a von-Neumann solution of a slightly perturbed zero-sum game. Our convergence guarantees are non-local, which as far as we know is a first-of-its-kind type of result in non-convex non-concave games. Finally, we discuss connections of our framework with generative adversarial networks.

==> Notes.tex <==
1. Maybe change title (NO DEFINITE ARTICLES)
2. Expand on related work (especially compared to last neurips)
3. Discuss safety with non-technical terms
4. Talk about ``independent'' variables (maybe related to 3)
5. Revisit the latent games paper (George)
6. Alternate Figures/Revised Figure 
    i. Recurrence vs Convergence
    ii. Explain something from the setting similar to Volume arguments of other paper (Lyapunov)
    iii. Describe the setting of the problem
    iv. Example of safe vs unsafe via example (or maybe closer to Lemma 1)
7. Rethink Lemma 1 and connections to safety, range of values, invertibility
    i. Without Lemma maybe it sounds informal.
8. Rethink bottom up vs top down presentation of the discussion (Holistic approach from start to end)
    i. Why analysis of (strictly) convex concave is easy
        ia. Lyapunov function distance from equilibrium.
        ib. No computable form of the Lyapunov function which necessary non constructive arguments. (refer to the theorems)
    ii. Is it easy to push the analysis of stability, convergence from convex-concave to hidden?
        ia. What is the new Lyapunov function?
        ib. When are the results global? (Link it back to safety and importance of initialization)
    iii. Transfer maps between spaces which lead naturally to re-parametrization.
        ia. Native domain is convex-concave but dynamics happen in the hidden space.
        ib. We need a coupling lemma to understand the connection (refer to theorems)
        
        
        
        
        Peiramata
        Insights
        Pws tou fainetai ews twra
        an einai thema an pame stis 9sels
        

==> contents/figures.tex <==



==> contents/hamiltonian.tex <==
\subsection{Connections to Hamiltonian Gradient Descent}
In GANs numerous learning heuristics are being tested and explored. One technique that has particular interesting theoretical justification as well as practical performance is Hamiltonian Gradient Descent (HGD). Understanding the convergence guarantees for HGD is an open research question \cite{hamilton1,hgd2018,hamitlon3}. We provide some new justification about its success in GANs by provably establishing convergence of a modified version of HGD in a relatively simple but illustrative subclass of hidden convex concave games, namely two by two hidden bi-linear games. This class of games is fairly expressive. Despite the restriction of planar bi-linear competition in the output space, the hidden game can have an arbitrary number of variables in the parameter space.

In the hidden two by two bi-linear presented in \cite{vlatakis2019poincare}, we have two functions $f: \mathbb{R}^N \to [0,1]$ and $g: \mathbb{R}^M \to [0,1]$ and two constants $(p,q) \in (0,1)^2$ where $(p,q)$ is the fully mixed equilibrium of the bi-linear game. Without loss of generality, we are interested in solving
\begin{equation*} 
\min_{\btheta \in \mathbb{R}^M} \max_{\bphi \in \mathbb{R}^N} (f(\btheta) - p)(g(\bphi) - q) 
\end{equation*}
Defining $L(\btheta, \bphi) = (f(\btheta) - p)(g(\bphi) - q)$, we can write down the dynamics of HGD~\cite{hgd2018}:
\begin{equation} \label{eq:original-hgd}
    \begin{aligned}
    \dot{\btheta}& =  - \frac{1}{2}\nabla_{\btheta} \norm{\nabla_{\bphi}L(\btheta, \bphi)}^2 - \frac{1}{2}\nabla_{\btheta} \norm{\nabla_{\btheta}L(\btheta, \bphi)}^2\\
    \dot{\bphi} &=  - \frac{1}{2}\nabla_{\bphi} \norm{\nabla_{\btheta}L(\btheta, \bphi)}^2  - \frac{1}{2}\nabla_{\bphi} \norm{\nabla_{\bphi}L(\btheta, \bphi)}^2
    \end{aligned}
\end{equation}
Observe that the second term of each right hand side would be zero in a classical bi-linear game but involves second order derivatives of $f$ and $g$ in the case of hidden bi-linear games. To circumvent the complexities of the second order derivatives and mimic the classical bi-linear game we will study a modified version of \cref{eq:original-hgd}, namely: 
\begin{equation}\label{eq:hamiltonian}
    \begin{aligned}
        \dot{\btheta}& =  - \frac{1}{2}\nabla_{\btheta} \norm{\nabla_{\bphi}L(\btheta, \bphi)}^2  \quad \quad
        \dot{\bphi} &=  - \frac{1}{2}\nabla_{\bphi} \norm{\nabla_{\btheta}L(\btheta, \bphi)}^2  
    \end{aligned}
\end{equation}

Employing an analysis similar to the one in \cref{sec:strict}, we get the following convergence result: 
\begin{theorem}\label{th:hamiltonian:main}
\input{contents/theorems/th_hamiltonian}
\end{theorem}

This convergence result is in stark contrast to the periodic trajectories of GDA analyzed by \cite{vlatakis2019poincare}.



==> contents/intro.tex <==
%%%% INTRO %%%%
%New Intro ??
% Global Lyapunov function in non-convex non-concave game dynamics
% Nash equilibria vs. 

% Other potential titles?
% 




\begin{comment}

\begin{itemize}
    \item {\bf Here is a problem.} 
     Understanding the behavior of learning dynamics in non-convex non-concave zero-sum games.
    \item {\bf It is an important problem.}
      A lot of applications. E.g. related to GANs but also AlphaGo/AlphaZero. 
      Also a question of historical importance. 
      Can von Neumann's fundamental theorem can in some sense be extended?
    \item {\bf It is an unsolved problem.}
    Even in very simple settings (e.g. a bilinear zero-sum game) game dynamics can have a complex behavior. 
    
    %understand stability/instability there. Carry over intuition to GANs experimentally.
    %Problem of approach one does not deal with the effects of deepnetworks. Too much of a toy.
    
     Recent interest in larger class of zero-sum games (e.g. truly general non-convex non-concave games, convex non-concave etc) and try to a) define a meaningful solution concept b) develop a dynamic that implements it.
    Problem of approach two, no true convergence results. This needs to be expanded more\dots
    
    
    \item {\bf Here is our solution.}
    We define the class of hidden/operator convex-concave games. They capture two critical aspects of the GANs. At the output level the games are convex-concave and admit a natural prescribed solution, the von-Neumann solution of the game. At the input level more Nash equilbria emerge (possibly infinitely many/continuums). The power of deepnetworks is also their curse. 
    A lot of phantom Nash equilibria (artifact of the nonlinearities) but effectively a unique Nash.
    
   \item {\bf Our solution works.}
   
Interaction Matters: A Note on Non-asymptotic Local Convergence of Generative Adversarial Networks Tengyuan Liang James Stokes AISTATS 2019
   
\end{itemize}

\end{comment}


\begin{comment}

NOTES to consider: 
1. Maybe change title (NO DEFINITE ARTICLES)
2. Expand on related work (especially compared to last neurips)
3. Discuss safety with non-technical terms
4. Talk about ``independent'' variables (maybe related to 3)
5. Revisit the latent games paper (George)
6. Alternate Figures/Revised Figure 
    i. Recurrence vs Convergence
    ii. Explain something from the setting similar to Volume arguments of other paper (Lyapunov)
    iii. Describe the setting of the problem
    iv. Example of safe vs unsafe via example (or maybe closer to Lemma 1)
7. Rethink Lemma 1 and connections to safety, range of values, invertibility
    i. Without Lemma maybe it sounds informal.
8. Rethink bottom up vs top down presentation of the discussion (Holistic approach from start to end)
    i. Why analysis of (strictly) convex concave is easy
        ia. Lyapunov function distance from equilibrium.
        ib. No computable form of the Lyapunov function which necessary non constructive arguments. (refer to the theorems)
    ii. Is it easy to push the analysis of stability, convergence from convex-concave to hidden?
        ia. What is the new Lyapunov function?
        ib. When are the results global? (Link it back to safety and importance of initialization)
    iii. Transfer maps between spaces which lead naturally to re-parametrization.
        ia. Native domain is convex-concave but dynamics happen in the hidden space.
        ib. We need a coupling lemma to understand the connection (refer to theorems)

\end{comment}
Traditionally, our understanding of zero-sum games revolves around von Neumann's celebrated minimax theorem which states:
Let $X \subset \mathbb{R}^n$ and $Y \subset \mathbb{R}^m$ be convex compact sets, if $L: X \times Y \rightarrow \mathbb{R}$ is a continuous convex-concave function, i.e., $L(\cdot,y):X\rightarrow\mathbb{R}$ is convex for fixed $y$, and $L(x,\cdot):Y\rightarrow\mathbb{R}$ is concave for fixed $x$  then we have that
\begin{equation} 
\tag{Convex-Concave}
\min_{x\in X}\max_{y\in Y} L(x,y) =\max_{y\in Y}\min_{x\in X}L(x,y)\\
\end{equation}
A pair $(x^*,y^*)$ is a \textit{(von Neumann) solution} to the min-max problem if and only if $x^*\in \argmin_{x\in X}\max_{y\in Y} L(x,y)$ and $y^* \in  \argmax_{y\in Y}\min_{x\in X}L(x,y)$.
\begin{comment}
Traditionally, our understanding of min-max (zero-sum) games revolves around von Neumann's celebrated minimax theorem which (under convexity/concavity conditions) guarantees the existence of a solution 
%
%Let $X \subset \mathbb{R}^n$ and $Y \subset \mathbb{R}^m$ be convex compact sets, if $L: X \times Y \rightarrow \mathbb{R}$ is a continuous convex-concave function, i.e., $L(\cdot,y):X\rightarrow\mathbb{R}$ is convex for fixed $y$, and $L(x,\cdot):Y\rightarrow\mathbb{R}$ is concave for fixed $x$  then we have that
%
%\begin{equation} 
%\tag{Convex-Concave}
%\min_{x\in X}\max_{y\in Y} L(x,y) =\max_{y\in Y}\min_{x\in X}L(x,y)\\
%\end{equation}
%
%
%
 $(x^*,y^*)$ 
%is a \textit{(von Neumann) solution} to the min-max problem if and only if 
 with
$x^*\in
\argmin_{x\in X}\max_{y\in Y} L(x,y)$ and $y^* \in  \argmax_{y\in Y}\min_{x\in X}L(x,y)$.
\end{comment}
This solution concept has a number of highly desirable properties. Even if multiple solutions exist, they all guarantee the same value for the agents. Any standard regret minimization algorithm suffices to compute them via time averaging of trajectories~\cite{Cesa06}. Recently more optimized techniques and analyses have produced multiple strong convergence results in these settings such as faster regret minimization rates or convergence of the day-to-day behavior~\cite{abernethy2018faster,yang2014regret,mertikopoulos2019optimistic,rakhlin2013online,wang2018acceleration,abernethy2019last,bailey2019finite,daskalakis2018training,daskalakis2018last,bailey2019fast,bailey2019finite,gidel2019a}.
\begin{comment}
%{\color{red}
%The renewed interest in min-max optimization has been largely motivated by the advent of Generative Adversarial Networks (GANs) and their numerous applications \cite{gan,radford2015unsupervised,salimans2016improved,isola2017image,zhang2017stackgan,arjovsky2017wasserstein,ledig2017photo}. GANs as a machine learning architecture is centered around the min-max competition between two agents, the generator and the discriminator. The generator aims to train a neural network that can generate high fidelity samples from a target distribution. The discriminator, on the other hand, seeks to train a neural network classifier than can distinguish between the artificially generated samples and those coming from the actual target distribution.}
%
Recently, min-max optimization has received renewed interest thanks to Generative Adversarial Networks (GANs) and their applications
\cite{gan,radford2015unsupervised,salimans2016improved,isola2017image,zhang2017stackgan,arjovsky2017wasserstein,ledig2017photo,WenRS19,YoonJS19,HwangJY19}.
GAN architectures revolve around the min-max competition between two agents, a generator and a discriminator. The generator fits a generative model aiming to produce samples from a target distribution while the discriminator trains a classifier to distinguish between real and synthesized samples. It is the antagonism from the discriminator that leads to better generators and the authentic looking samples from the generator that lead to better discriminators.   



One of the key limitations of GANs is that training them can be notoriously difficult and unstable \cite{salimans2016improved,mertikopoulos2018cycles,kodali2017convergence,cheung2019vortices,vlatakis2019poincare}. Addressing this limitation has been the object of intensive  investigation \cite{radford2015unsupervised,mescheder2018training,metz2016unrolled,pfau2016connecting,tolstikhin2017adagan,berthelot2017began,gulrajani2017improved,balduzzi2018mechanics,yazici2018unusual,2020arXiv200208456P}. The development of numerous interesting heuristics, however, while useful from a practical perspective has created a fragmented picture with no clear and concise theoretical insights  at the polar opposite of the clarity of von Neumann's theorem.

Naturally, this complexity is to some extent unavoidable as  
% A core obstacle in this direction is that, despite the self-evident min-max nature of the competition between generator and discriminator, 
 the introduction of deep networks in GANs pushes us away from the safe shore of convex-concave games. 
 \end{comment}
 
When we venture beyond the well-trodden paths of convex-concave games, von Neumann's theorem no longer applies and it is not even clear what constitutes a meaningful solution point.  The function $L$ may have numerous local saddle/Nash points 
 %(or even global ones)\footnote{These are points in the parameter space such that no agent can improve their performance via local/global deviations respectively.}
 that result in widely different values for the agents. 
 %To address this important limitation of local Nash, 
 \begin{comment}
 The lack of clarity is further intensified when taking the learning dynamics into account.
 \end{comment} 
 Distressingly, in general min-max games there exist stable fixed points for standard optimization driven dynamics that are not even local Nash and are thus clearly undesirable from a game theoretic perspective~\cite{mazumdar2018convergence,adolphs2018local,daskalakis2018limit}. 
 %Is it possible to somehow circumvent all these negatives results and create a theoretical underpinning of  that mirrors our clear-cut understanding of classic zero-sum games?
 
  Different solutions concepts have been proposed such as local max-min (local min-max), Stackleberg equilibria %that order agents and e.g, give the first order move opportunity to the max-agent/min-agent 
 \cite{jin2019minmax,fiez2019convergence,2020arXiv200211875Z} or resource-bounded Nash equilibria~\cite{oliehoek2018beyond}. 
%or even infinitely dimensional extensions of Nash equilibria~\cite{hsieh2018finding}. 
 However, \note{understanding which type of equilibrium is selected by standard optimization methods like  gradient-descent-ascent (GDA) is still an unresolved issue.}
 
 
{\bf Is it possible to define a class of non-convex non-concave games with an effectively unique game theoretic solution that is selected by standard dynamics (e.g. gradient descent)?}

 
{\bf Our class of games.} We will define a general class of min-max optimization problems, 
%that includes all convex-concave games but at the same time critically captures key features of the GAN framework. 
 where 
 each agent selects its own vectors of parameters which are then processed separately by smooth functions. Each agent  receives their respective payoff after entering the outputs of  the processed decision vectors as inputs to a standard convex-concave game. Formally,  there exist functions $\bF: \mathbb{R}^{N} \to X \subset \mathbb{R}^{n}$ and $\bG: \mathbb{R}^{M} \to Y \subset \mathbb{R}^{m}$ and  a continuous convex-concave function $L: X \times Y \rightarrow \mathbb{R}$, such that the min-max game is 

\begin{equation*} 
\label{eq:min-max}
%(\btheta^*,\bphi^*) = 
\min_{\btheta \in \mathbb{R}^{N}}\max_{\bphi \in \mathbb{R}^{M}} L(\bF(\btheta) ,\bG(\bphi)). \tag{ Hidden Convex-Concave  (HCC)}
\end{equation*}

We call this class of min-max problems Hidden Convex-Concave Games. It generalizes the recently defined hidden bilinear games of ~\cite{vlatakis2019poincare}. 
%Clearly, 
%the proposed class of games is  directly inspired by  GANs. During GAN training the discriminator and the generator input their chosen parameters, denoted as  $\pmb{\theta}$ and $\pmb{\phi}$ in our formulation, to their neural networks. Deepnets introduce nonlinearities as they map these parameters to their output space.
%In our setting this is captured via the non-convex functions $F, G$. 
%Critically, and unlike~\cite{vlatakis2019poincare}, we will allow for general convex-concave competition on the output space. This will be instrumental both in terms of capturing standard GANs formulations (see \cref{sec:ganconnections}), as well as in showing that the cyclic behavior reported in~\cite{vlatakis2019poincare} corresponds to an edge case that can be circumvented to provide strong convergence results. 

{\bf Our solution concept.} Out of all the local Nash equilibria of HCC games, there exists a special subclass, the vectors $(\btheta^*,\bphi^*)$ that implement the von Neumann solution of the convex-concave games. This solution has a  strong and intuitive game theoretic justification. Indeed, it is stable even if the agents could  perform arbitrary deviations directly on the output spaces $X, Y$. These parameter combinations $(\btheta^*,\bphi^*)$ ``solve" the ``hidden" convex-concave $L$ and thus we call them \textit{von Neumann solutions}. Naturally, HCCs will typically have numerous local saddle/Nash equilibria that do not satisfy this property. Instead, they correspond to stationary points of the $\bF, \bG$ where their output is stuck, e.g., due to an unfortunate initialization. At these points the agents may be receiving payoffs which can be arbitrarily smaller/larger than the game theoretic value of game $L$. 
%They do not represent any meaningful information about the game. Instead, they are merely an artifact introduced by the non-linear operators. 
\note{Fortunately, we show that GDA favors von Neumann solutions that are feasible for a given initialization.}
%typically only the von Neumann solutions will arise naturally.
%do not merely have a  much stronger game theoretic justification than local Nash equilibria but also from an algorithmic one. 
  %We would like to create a class of non-convex non-concave game that captures the key elements of GANs, that has a well defined solution that agrees with pre-existing analysis of GANs and for which standard optimization dynamics give strong evidence in favor of.
%On gradient descent ascent for nonconvex-concave minimax problems
%T Lin, C Jin, MI Jordan - arXiv preprint arXiv:1906.00331, 2019 - arxiv.org
% Solving a class of non-convex min-max games using iterative first order methods
%M Nouiehed, M Sanjabi, T Huang, JD Lee, M Razaviyayn
%Advances in Neural Information Processing Systems, 14905-14916
%, however, these solutions
%do not address the issue of equilibrium selection. 
%1. zeros-sum games that admit non-Nash attracting equilibria of the gradient dynamics. Such points are attracting under the learning dynamics, yet at least one player—and potentially all of them—has a direction in which they could unilaterally deviate to decrease their cost. Thus, these non-Nash equilibria
%3. Undesirable stable stationary points for GD in non-convex non-concave games that are no local optima
%Min-max optimization formulations make for natural models of this competition and have been employed in the study of multiple GAN related issues \cite{arora2017generalization,ma2018generalization,yazici2018unusual,ge2018fictitious}.
%The %min-max co-evolution of both agents has been at the core of success of GANs.
%Machine Learning researchers and practitioners have tried to formalize this competition using the min-max optimization framework mentioned above with great success \cite{arora2017generalization,ma2018generalization,ge2018fictitious,yazici2018unusual}.
%Critically, however, when we move away from the standard class of convex-concave to general non-convex non-concave zero-sum games, 













































\begin{comment}
In this work, we present a global analysis of the
stability and the convergence properties of gradient descent-ascent (GDA) 
dynamics for a wide class of non-convex non-concave zero-sum games which by design
incorporates hidden strong convexity structure as well as of single-agent non-convex optimization. 
Our workhorse is motivated by the {\cite{OurNIPS19}}'s model where the two players control the input vectors $(\pmb{\theta}:\text{min-player},\pmb{\phi}:\text{max-player})$ of smooth functions whose outputs $F(\pmb{\theta}),G(\pmb{\phi})$ are being applied to a general non-convex non-concave min-max optimization objective $u\left(F(\pmb{\theta}),G(\pmb{\phi})\right)$ under a smooth version of (GDA) described by a dynamical
system in continuous time. 

Informally, we prove that for this class of hidden games convergence to a Von-Neumann solution is tractable by GDA dynamics, subverting the established expectations, when a specific intrinsic strong convex-concave decomposition of utility function is possible. Additionally, we present how classical regularization techniques can be applied in the hidden games, which lack the strong notion of convexity properties like bi-linear games, to converge to a slightly perturbed Nash equilibrium. Finally in order to explore the implications of our results, we investigate their application to the main variations of GANs (\textit{vanilla},\textit{f-GAN},\textit{WGAN}). On the other side of the coin, we complete our analysis by presenting counter-examples which yield the necessity of any safety initial conditions that we assert in our positive results.  

From a technical point of view, our analysis touches on several issues. Initially,
leveraging the reparametrization machinery of {\cite{OurNIPS19}} we state an equivalence from the parameter space $(\theta,\phi)$ to the induced dynamics of functional space $(F,G)$...
1) Stability of the Saddle points set \\
2) Strictness of either convex or concave part implies asympotic stability and convergence to a single
fixed point\\
3) Prove that Hamiltonian plays an underlying role of a norm \\
4) Exploiting (3) transfer (1) and (2) to the original parametrical space
5) For the non-strict case, regularization scheme are possible. In the illustrative 2x2 example
Hamiltonian Descent can be applied.\\
6) Parity function is a tight example for the safety conditions.

%More formally, we first show that ordinary "vanilla" GDA converges under a strong convexity condition of hidden games. Additionally, we analyze the asymptotic stability of the fixed points of GDA Dynamics

%,
%we are able to show that having a utility function $u(F(\pmb{x}),G(\pmb{y})$
%which



So, we firstly derived the equivalent (``topological conjugate'') system of GDA dynamics in the output space. 
Despite the non-inversibility of the operators, this is actually possible after an intricate study of 
a time-varying modification of the gradient ascent (Theorem ??). 
\end{comment}

%\textit{Connection with GANs.} Critically, the dynamics act on the input/parameter space $\btheta,\bphi$ of non convex-operators $(\bF,\bG)$, instead of accessing directly the output space $L(\bF(\btheta),\bG(\bphi))$. Thus, thanks to this indirect competition, we are able to show that the expressivity of this family of games incorporates fully the vast majority of the proposed GANs architectures. More surprisingly, instead of focusing in different notions of equilibrium, from the hidden convex-concave viewpoint  min-max optima of GANs architectures correspond to the old-fashioned Von Neumann's solution (\Cref{sec:??}). 

%Lyapunov stability does not suffice to prove directly pointwise convergence to a Von Neumann's solution.
%Additionally, \cite{vlatakis2019poincare} showed that the hidden bi-linear case is always cycling around the equilibrium.

%Intuitively we would like  to leverage the underlying convex-concave properties of the operators. 
\begin{comment}
\begin{itemize}
    \item {\bf Here is a problem.} 
    %Why GANs work so well? Why GANs sometimes fail?
    \item {\bf It is an important problem.}
      A lot of applications. Connections with the fundamental game theoretic concept of zero-sum games. 
    \item {\bf It is an unsolved problem.}
    Two types of approaches at a high level.
    Approach one: Approximate GANs with a much simpler setting (e.g. a bilinear zero-sum game) understand stability/instability there. Carry over intuition to GANs experimentally.
    Problem of approach one does not deal with the effects of deepnetworks. Too much of a toy.
    
    Approach two: Consider a much larger class of zero-sum games (e.g. truly general non-convex non-concave games, convex non-concave etc) and try to a) define a meaningful solution concept b) develop a dynamic that implements it.
    Problem of approach two, no true convergence results. Not clear if solution concept is a good match for GANs.
    
    \item {\bf Here is our solution.}
    We define the class of hidden/operator convex-concave games. They capture two critical aspects of the GANs. At the output level the games are convex-concave and admit a natural prescribed solution, the von-Neumann solution of the game. At the input level more Nash equilbria emerge (possibly infinitely many/continuums). The power of deepnetworks is also their curse. 
    A lot of phantom Nash equilibria (artifact of the nonlinearities) but effectively a unique Nash.
    
   \item {\bf Our solution works.}
   
Interaction Matters: A Note on Non-asymptotic Local Convergence of Generative Adversarial Networks Tengyuan Liang James Stokes AISTATS 2019
   
\end{itemize}
\end{comment}

==> contents/intro2.tex <==
%%%% INTRO %%%%
%New Intro ??
% Global Lyapunov function in non-convex non-concave game dynamics
% Nash equilibria vs. 

% Other potential titles?
% 




\begin{comment}

\begin{itemize}
    \item {\bf Here is a problem.} 
     Understanding the behavior of learning dynamics in non-convex non-concave zero-sum games.
    \item {\bf It is an important problem.}
      A lot of applications. E.g. related to GANs but also AlphaGo/AlphaZero. 
      Also a question of historical importance. 
      Can von Neumann's fundamental theorem can in some sense be extended?
    \item {\bf It is an unsolved problem.}
    Even in very simple settings (e.g. a bilinear zero-sum game) game dynamics can have a complex behavior. 
    
    %understand stability/instability there. Carry over intuition to GANs experimentally.
    %Problem of approach one does not deal with the effects of deepnetworks. Too much of a toy.
    
     Recent interest in larger class of zero-sum games (e.g. truly general non-convex non-concave games, convex non-concave etc) and try to a) define a meaningful solution concept b) develop a dynamic that implements it.
    Problem of approach two, no true convergence results. This needs to be expanded more\dots
    
    
    \item {\bf Here is our solution.}
    We define the class of hidden/operator convex-concave games. They capture two critical aspects of the GANs. At the output level the games are convex-concave and admit a natural prescribed solution, the von-Neumann solution of the game. At the input level more Nash equilbria emerge (possibly infinitely many/continuums). The power of deepnetworks is also their curse. 
    A lot of phantom Nash equilibria (artifact of the nonlinearities) but effectively a unique Nash.
    
   \item {\bf Our solution works.}
   
Interaction Matters: A Note on Non-asymptotic Local Convergence of Generative Adversarial Networks Tengyuan Liang James Stokes AISTATS 2019
   
\end{itemize}

\end{comment}


\begin{comment}

NOTES to consider: 
1. Maybe change title (NO DEFINITE ARTICLES)
2. Expand on related work (especially compared to last neurips)
3. Discuss safety with non-technical terms
4. Talk about ``independent'' variables (maybe related to 3)
5. Revisit the latent games paper (George)
6. Alternate Figures/Revised Figure 
    i. Recurrence vs Convergence
    ii. Explain something from the setting similar to Volume arguments of other paper (Lyapunov)
    iii. Describe the setting of the problem
    iv. Example of safe vs unsafe via example (or maybe closer to Lemma 1)
7. Rethink Lemma 1 and connections to safety, range of values, invertibility
    i. Without Lemma maybe it sounds informal.
8. Rethink bottom up vs top down presentation of the discussion (Holistic approach from start to end)
    i. Why analysis of (strictly) convex concave is easy
        ia. Lyapunov function distance from equilibrium.
        ib. No computable form of the Lyapunov function which necessary non constructive arguments. (refer to the theorems)
    ii. Is it easy to push the analysis of stability, convergence from convex-concave to hidden?
        ia. What is the new Lyapunov function?
        ib. When are the results global? (Link it back to safety and importance of initialization)
    iii. Transfer maps between spaces which lead naturally to re-parametrization.
        ia. Native domain is convex-concave but dynamics happen in the hidden space.
        ib. We need a coupling lemma to understand the connection (refer to theorems)

\end{comment}
Traditionally, our understanding of zero-sum games revolves around von Neumann's celebrated minimax theorem which states:
Let $X \subset \mathbb{R}^n$ and $Y \subset \mathbb{R}^m$ be convex compact sets, if $L: X \times Y \rightarrow \mathbb{R}$ is a continuous convex-concave function, i.e., $L(\cdot,y):X\rightarrow\mathbb{R}$ is convex for fixed $y$, and $L(x,\cdot):Y\rightarrow\mathbb{R}$ is concave for fixed $x$  then we have that
\begin{equation} 
\tag{Convex-Concave}
\min_{x\in X}\max_{y\in Y} L(x,y) =\max_{y\in Y}\min_{x\in X}L(x,y)\\
\end{equation}
A pair $(x^*,y^*)$ is a \textit{(von Neumann) solution} to the min-max problem if and only if $x^*\in \argmin_{x\in X}\max_{y\in Y} L(x,y)$ and $y^* \in  \argmax_{y\in Y}\min_{x\in X}L(x,y)$.
\begin{comment}
Traditionally, our understanding of min-max (zero-sum) games revolves around von Neumann's celebrated minimax theorem which (under convexity/concavity conditions) guarantees the existence of a solution 
%
%Let $X \subset \mathbb{R}^n$ and $Y \subset \mathbb{R}^m$ be convex compact sets, if $L: X \times Y \rightarrow \mathbb{R}$ is a continuous convex-concave function, i.e., $L(\cdot,y):X\rightarrow\mathbb{R}$ is convex for fixed $y$, and $L(x,\cdot):Y\rightarrow\mathbb{R}$ is concave for fixed $x$  then we have that
%
%\begin{equation} 
%\tag{Convex-Concave}
%\min_{x\in X}\max_{y\in Y} L(x,y) =\max_{y\in Y}\min_{x\in X}L(x,y)\\
%\end{equation}
%
%
%
 $(x^*,y^*)$ 
%is a \textit{(von Neumann) solution} to the min-max problem if and only if 
 with
$x^*\in
\argmin_{x\in X}\max_{y\in Y} L(x,y)$ and $y^* \in  \argmax_{y\in Y}\min_{x\in X}L(x,y)$.
\end{comment}
This solution concept has a number of highly desirable properties. Even if multiple solutions exist, they all guarantee the same value for the agents. Any standard regret minimization algorithm suffices to compute them via time averaging of trajectories~\cite{Cesa06}. Recently more optimized techniques and analyses have produced multiple strong convergence results in these settings such as faster regret minimization rates or convergence of the day-to-day behavior~\cite{abernethy2018faster,yang2014regret,mertikopoulos2019optimistic,rakhlin2013online,wang2018acceleration,abernethy2019last,bailey2019finite,daskalakis2018training,daskalakis2018last,bailey2019fast,bailey2019finite,gidel2019a}.
\begin{comment}
%{\color{red}
%The renewed interest in min-max optimization has been largely motivated by the advent of Generative Adversarial Networks (GANs) and their numerous applications \cite{gan,radford2015unsupervised,salimans2016improved,isola2017image,zhang2017stackgan,arjovsky2017wasserstein,ledig2017photo}. GANs as a machine learning architecture is centered around the min-max competition between two agents, the generator and the discriminator. The generator aims to train a neural network that can generate high fidelity samples from a target distribution. The discriminator, on the other hand, seeks to train a neural network classifier than can distinguish between the artificially generated samples and those coming from the actual target distribution.}
%
Recently, min-max optimization has received renewed interest thanks to Generative Adversarial Networks (GANs) and their applications
\cite{gan,radford2015unsupervised,salimans2016improved,isola2017image,zhang2017stackgan,arjovsky2017wasserstein,ledig2017photo,WenRS19,YoonJS19,HwangJY19}.
GAN architectures revolve around the min-max competition between two agents, a generator and a discriminator. The generator fits a generative model aiming to produce samples from a target distribution while the discriminator trains a classifier to distinguish between real and synthesized samples. It is the antagonism from the discriminator that leads to better generators and the authentic looking samples from the generator that lead to better discriminators.   



One of the key limitations of GANs is that training them can be notoriously difficult and unstable \cite{salimans2016improved,mertikopoulos2018cycles,kodali2017convergence,cheung2019vortices,vlatakis2019poincare}. Addressing this limitation has been the object of intensive  investigation \cite{radford2015unsupervised,mescheder2018training,metz2016unrolled,pfau2016connecting,tolstikhin2017adagan,berthelot2017began,gulrajani2017improved,balduzzi2018mechanics,yazici2018unusual,2020arXiv200208456P}. The development of numerous interesting heuristics, however, while useful from a practical perspective has created a fragmented picture with no clear and concise theoretical insights  at the polar opposite of the clarity of von Neumann's theorem.

Naturally, this complexity is to some extent unavoidable as  
% A core obstacle in this direction is that, despite the self-evident min-max nature of the competition between generator and discriminator, 
 the introduction of deep networks in GANs pushes us away from the safe shore of convex-concave games. 
 \end{comment}
 
When we venture beyond the well-trodden paths of convex-concave games, von Neumann's theorem no longer applies and it is not even clear what constitutes a meaningful solution point.  The function $L$ may have numerous local saddle/Nash points 
 %(or even global ones)\footnote{These are points in the parameter space such that no agent can improve their performance via local/global deviations respectively.}
 that result in widely different values for the agents. 
 %To address this important limitation of local Nash, 
 \begin{comment}
 The lack of clarity is further intensified when taking the learning dynamics into account.
 \end{comment} 
 Distressingly, in general min-max games there exist stable fixed points for standard optimization driven dynamics that are not even local Nash and are thus clearly undesirable from a game theoretic perspective~\cite{mazumdar2018convergence,adolphs2018local,daskalakis2018limit}. 
 %Is it possible to somehow circumvent all these negatives results and create a theoretical underpinning of  that mirrors our clear-cut understanding of classic zero-sum games?
 
  Different solutions concepts have been proposed such as local max-min (local min-max), Stackleberg equilibria %that order agents and e.g, give the first order move opportunity to the max-agent/min-agent 
 \cite{jin2019minmax,fiez2019convergence,2020arXiv200211875Z} or resource-bounded Nash equilibria~\cite{oliehoek2018beyond}. 
%or even infinitely dimensional extensions of Nash equilibria~\cite{hsieh2018finding}. 
 However, \note{understanding which type of equilibrium is selected by standard optimization methods like  gradient-descent-ascent (GDA) is still an unresolved issue.}
 
 
{\bf Is it possible to define a class of non-convex non-concave games with an effectively unique game theoretic solution that is selected by standard dynamics (e.g. gradient descent)?}

 
{\bf Our class of games.} We will define a general class of min-max optimization problems, 
%that includes all convex-concave games but at the same time critically captures key features of the GAN framework. 
 where 
 each agent selects its own vectors of parameters which are then processed separately by smooth functions. Each agent  receives their respective payoff after entering the outputs of  the processed decision vectors as inputs to a standard convex-concave game. Formally,  there exist functions $\bF: \mathbb{R}^{N} \to X \subset \mathbb{R}^{n}$ and $\bG: \mathbb{R}^{M} \to Y \subset \mathbb{R}^{m}$ and  a continuous convex-concave function $L: X \times Y \rightarrow \mathbb{R}$, such that the min-max game is 
\begin{equation*} 
\label{eq:min-max}
\min_{\btheta \in \mathbb{R}^{N}}\max_{\bphi \in \mathbb{R}^{M}} L(\bF(\btheta) ,\bG(\bphi)). \tag{ Hidden Convex-Concave  (HCC)}
\end{equation*}
We call this class of min-max problems Hidden Convex-Concave Games. It generalizes the recently defined hidden bilinear games of ~\cite{vlatakis2019poincare}.

{\bf Our solution concept.} Out of all the local Nash equilibria of HCC games, there exists a special subclass, the vectors $(\btheta^*,\bphi^*)$ that implement the von Neumann solution of the convex-concave games. This solution has a  strong and intuitive game theoretic justification. Indeed, it is stable even if the agents could  perform arbitrary deviations directly on the output spaces $X, Y$. These parameter combinations $(\btheta^*,\bphi^*)$ ``solve" the ``hidden" convex-concave $L$ and thus we call them \textit{von Neumann solutions}. Naturally, HCCs will typically have numerous local saddle/Nash equilibria that do not satisfy this property. Instead, they correspond to stationary points of the $\bF, \bG$ where their output is stuck, e.g., due to an unfortunate initialization. At these points the agents may be receiving payoffs which can be arbitrarily smaller/larger than the game theoretic value of game $L$. 
\note{Fortunately, we show that GDA favors von Neumann solutions that are feasible for a given initialization.}


\textbf{Our results.} \note{In this work, we study the behavior of continuous GDA dynamics for the class of HCC games where each coordinate of $\bF,\bG$ is controlled by disjoint sets of variables. In a nutshell, we show that GDA trajectories stabilize around or converge to the corresponding von Neumann solutions of the hidden game. Despite restricting our attention to a subset of HCC games, our analysis has to overcome unique hurdles not shared by standard convex concave games.

\textit{Challenges of HCC games. }In convex-concave games, deriving the stability of the von Neumann solutions
relies on the Euclidean distance from the equilibrium being a Lyapunov function. 
In contrast, in HCC games where optimization happens in the parameter space of $\btheta,\bphi$, the non-linear nature of $\bF,\bG$ distorts the convex-concave landscape in the output space. Thus, the Euclidean distance can not be in general a Lyapunov function. In addition , the existence of a Lyapunov function for the trajectories in the output space of $\bF,\bG$
would not imply the existence of a Lyapunov function in the parameter space unless $\bF,\bG$ were invertible maps.
Even if $L$ has a unique solution in the output space, this solution could be implemented by multiple equilibria 
in the parameter space and thus each of them can not be individually globally attracting. Clearly any transfer of stability or
convergence properties from the output to the parameter space needs to be initialization dependent.

%This does not extend generally 
%to HCC games.
%initialization specifics one to one mapping
%Lyapunov functions

\textit{Lyapunov Stability.} 
Our first step is to construct an initialization-dependent Lyapunov function that accounts for the curvature induced by the operators $\bF$ and $\bG$ (\Cref{lemma:lyapunov-function}). Leveraging a potentially infinite number of initialization-dependent Lyapunov functions in \cref{th:hidden_meta_stability}  we prove that under mild assumptions the outputs of $\bF,\bG$ stabilize around the von Neumann solution of $L$. 
%Combining potentially an infinite number of initialization-dependent Lyapunov functions necessitates a detailed analysis of 
%techniques beyond what is required for the standard convex-concave games.
%To achieve this result, a detailed analysis is necessary of possibly infinite number of different Lyapunov functions
%This is surpiring given 
%despite the euclidean distance
%from a von Neumann solution in the output space may increase, 
%In \Cref{th:stability_sigmoid_main,th:hidden_meta_stability} we describe sufficient conditions 
%for the the operators space $\bF,\bG$ that allow us to transfers stability properties to the space of the parameters $\btheta$ and $\bphi$.\\
%present how this notion of stability in the operators space $\bF,\bG$ transfers back to the space of the parameters $\btheta$ and $\bphi$.
%(\Cref{th:conv-conc-transformed})
%thereof
%Our first step is to prove that under GDA dynamics in HCC games von Neumann solutions are stable in the output space. 
%In order to establish that, we construct a Lyapunov function tailored to our setting. In contrast with the standard convex-concave min-max games, hidden structure poses distinct hurdles. While in the fundamental case of convex concave games, the distance from the von Neuman solution acts as a potential function, in HCC games this is no longer the case. To sidestep this issue,
%To prove this, we construct a Lyapunov function that accounts for the curvature induced by the operators $\bF$ and $\bG$ (\Cref{th:conv-conc-transformed}). In \Cref{th:stability_sigmoid_main,th:hidden_meta_stability}  we present how this notion of stability in the operators space $\bF,\bG$ transfers back to the space of the parameters $\btheta$ and $\bphi$.
%On the other hand we don't restrict the operators $\bF,\bG$, retaining the non-convex non-concave nature of the composite game. 
%using the implications of LaSalle's Invariance Principle we are able to obtain
%In the case of strict-HCC games 

\textit{Convergence.}
Mirroring convex concave games, we require strict convexity or concavity of $L$ to provide convergence guarantees 
 to von Neumann solutions (\Cref{th:strict-convergence}). Barring initializations where von Neumann solutions are not reachable due to the limitations imposed by $\bF$ and $\bG$, the set of von Neumann solutions are globally asymptotically stable (\Cref{cor:global-conv}).
Even in non-strict HCC games,  we can add regularization terms to make  $L$ strictly convex concave. Small amounts of regularization allows for convergence without significantly perturbing the von Neumann solution (\Cref{th:regularization:main}) while increasing regularization enables exponentially faster convergence rates (\Cref{th:regularization:rate}). %For the special but illustrative case of 2x2 hidden bi-linear games, that are not strictly HCC, we can achieve convergence (\Cref{th:hamiltonian:main}) to the unperturbed solution by employing a modification of the Hamiltonian Gradient Descent dynamics \cite{hgd2018}.
}


==> contents/related.tex <==
{\color{red}Related work?}


==> contents/results.tex <==


\textbf{Our results.} We prove that GDA for the class of hidden convex concave games stabilize or converge around the corresponding von Neumann solutions of the hidden game. In a nutshell, this work presents a new class of non-convex non-concave min-max games for which continuous dynamics of gradient flows exhibit both Lyapunov stability and under mild assumptions actually converge to the desired von Neumann solution. 

\textit{Lyapunov Stability.} Our first step is to prove that under GDA dynamics in HCC games von Neumann solutions are stable. In order to establish that, we construct a Lyapunov function tailored to our setting. In contrast with the standard convex-concave min-max games, hidden structure poses distinct hurdles. While in the fundamental case of convex concave games, the distance from the von Neuman solution acts as a potential function, in HCC games this is no longer the case. To sidestep this issue, we construct a Lyapunov function that accounts for the curvature induced by the operators $\bF$ and $\bG$ (\Cref{th:conv-conc-transformed}). In \Cref{th:stability_sigmoid_main,th:hidden_meta_stability}  we present how this notion of stability in the operators space $\bF,\bG$ transfers back to the space of the parameters $\btheta$ and $\bphi$.

\textit{Asymptotic Convergence.}
Mirroring the case of classical convex concave games, we require strict convexity or concavity of the hidden game to provide convergence guarantees. On the other hand we don't restrict the operators $\bF,\bG$, retaining the non-convex non-concave nature of the composite game. In \Cref{th:strict-convergence}, using the implications of LaSalle's Invariance Principle we are able to obtain convergence guarantees to von Neumann solutions. Barring initializations where von Neumann solutions are not reachable due to the limitations imposed by $\bF$ and $\bG$, the set of von Neumann solutions are globally asymptotically stable (\Cref{cor:global-conv}).

\textit{Regularization }
Even in non-strict HCC games, however,  we can add regularization terms that make the hidden game strictly convex concave. Small amounts of regularization can allow for convergence without significantly perturbing the von Neumann solution (\Cref{th:regularization:main}) while increasing regularization allows for exponentially faster convergence (\Cref{th:regularization:rate}). %For the special but illustrative case of 2x2 hidden bi-linear games, that are not strictly HCC, we can achieve convergence (\Cref{th:hamiltonian:main}) to the unperturbed solution by employing a modification of the Hamiltonian Gradient Descent dynamics \cite{hgd2018}.



==> contents/tableGans.tex <==

\begin{table}[t!]
    \centering
    \begin{tabular}{c c c c} 
        \midrule
        Type of GAN & $G^*$ & $D^*$ &  Hidden Structure \\ [0.5ex] 
        \midrule \midrule 
        {\color{darkgreen}GAN}  & $p_{\textrm{data}}$ & $\tfrac{1}{2}$ & Linear VS Strongly-Concave \\ [1.ex] 
        {\color{darkred}GAN}& $\argmin_{G\in \mathcal{G}}\mathrm{JSD} (p_{\textrm{data}}||p_{\textrm{G}}) $ & $\tfrac{p_{\textrm{data}}}{p_{\textrm{data}}+p_{\textrm{G}^*}}$  & Linear VS Strongly-Concave\\ [1.ex]
        \midrule \midrule 
         {\color{darkgreen}f-GAN}  & $p_{\textrm{data}}$ & $f'(1)$  & Linear VS Concave \\ [1.ex] 
        {\color{darkred}f-GAN}& $\argmin_{G\in \mathcal{G}}\mathrm{D}_f (p_{\textrm{data}}||p_{\textrm{G}}) $ & $f'\left(\tfrac{p_{\textrm{data}}}{p_{\textrm{G}^*}}\right)$  & Linear VS Concave \\ [1.ex] 
        \midrule \midrule 
        {\color{darkgreen}WGAN}  & $p_{\textrm{data}}$ & $c$ & Linear VS Linear \\ [1.ex] 
        {\color{darkred}WGAN}& $\argmin_{G\in \mathcal{G}}\mathrm{EMD} (p_{\textrm{data}}||p_{\textrm{G}}) $ & \textendash\  & Linear VS Linear \\ [1.ex] 
        \midrule \midrule 
    \end{tabular}
    \caption{$p_{\textrm{data}}$ represents the target data distribution. $G^*$ is the min-max generator and $D^*$ is the max-min discriminator. $\mathrm{JSD}$ denotes the Jensen–Shannon divergence, $\mathrm{D}_f$ the $f$-divergence for the convex function $f$ and $\mathrm{EMD}$ the earth mover distance and $c$ the constant discriminator. {\color{darkgreen}xGAN}, {\color{darkred}xGAN} correspond to the {\color{darkgreen} realizable } and the {\color{darkred}non-realizable case } accordingly. \textendash\ indicates the lack of a closed form solution for $D^*$ of {\color{darkred}WGAN}.}
    \label{tab:my_label}
\end{table}


\subsection{Connections to GANs}\label{sec:ganconnections}
At the heart of many GAN formulations like the standard GAN \cite{gan}, f-GAN \cite{fgan} and Wassertein GAN (WGAN) \cite{wgan} lies a classical convex concave game in the operator output space. Indeed for the realizeable case \cite{gan} used the underlying convexity properties to find the Nash equilibria of standard GAN and \cite{gansmaynothavenash} did the same thing for the f-GAN and WGAN. Perhaps surprisingly, neither work references explicitly the convex concave nature of the operator output space game or von Neumann's minimax theorem. To highlight the significance of von Neumann equilibria as a solution concept for GANs, we show how  $G^*$ and $D^*$ of \cref{tab:my_label} can be derived separately from each other by solving the corresponding min-max (max-min) problems. This allows one to independently verify the validity of von Neumann's minimax theorem and its generalizations for GANs. We also extend our analysis to a wide class of non-realizeable cases as well. We defer the  theorem statements as well as their proofs to Appendix B. 

In practice however, as noted explicitly by \cite{DBLP:journals/corr/Goodfellow17}, the updates in GAN training happen in the parameter space giving rise to a HCC game. This has exactly inspired our proposed solution concept for GANs, generators and discriminators implementing a von Neumann solution of the underlying convex concave game. It also motivates studying the learning dynamics of HCC games in \cref{sec:results}.   





==> contents/theorems/cor_cc_stability.tex <==
Let $L$ is convex concave and  $(\bp, \bq) \in \saddle(L)$, then $(\bp, \bq)$ is stable for continuous GDA dynamics.
In other words, for every $\epsilon > 0$, there is an $\delta >0 $ such that
\begin{equation*}
    r(0) < \delta \implies \forall t\geq 0 : r(t) < \epsilon.
\end{equation*}
where
\begin{equation*}
   r(t) = \norm{\mathbf{x}(t) - \bp}^2 + \norm{\mathbf{y}(t) - \bq}^2. 
\end{equation*}


==> figures/model.tex <==

\tdplotsetmaincoords{70}{100}
\begin{tikzpicture}[tdplot_main_coords,scale=0.75]

\draw [<-,thick]  (5.5,4+4,4.5) to [in=-30,out=-150] (1,2,3) ;%(5,2) ;
\draw [<-,thick]  (5.5,4+4.5,4.5) to [in=-170,out=-30] (2,13.5,3) ;%(5,2) ;
\draw [->,thick]  (3.75,3.75,7) to [out=200,in=100] (1,2,3) ;%(5,2) ;
\draw [->,thick]  (3.75,3.75+10,7) to [out=250,in=100] (2,13.5,3) ;%(5,2) ;
\draw[<-,thick,orange] (2,13.8,6)-- (2,13.8,3) -- (4,13.8,3)--(4,7.75,3)--(1.75,7.75,3);
\draw[->,thick,orange] (1.75,7.5 ,3) -- (4,7.5,3)--(4,1.75,3)--(1.75,1.75,3)--(1.75,1.75,6); \def\offsetY{5}
\def\offsetX{0}
  \foreach\transferx in {0,10}
  {
  \foreach\latentz in {3,7}
    {
      \fill [opacity=.2,blue] (\offsetX,0+\transferx ,\latentz) -- (\offsetX+\offsetY,0+\transferx ,\latentz) --
        (\offsetX+\offsetY ,\offsetX+\offsetY+\transferx,\latentz) -- (\offsetX,\offsetX+\offsetY+\transferx ,\latentz) --cycle;
        \draw [opacity=.7,blue] (\offsetX,0+\transferx ,\latentz) -- (\offsetX+\offsetY,0+\transferx ,\latentz) --
        (\offsetX+\offsetY ,\offsetX+\offsetY+\transferx,\latentz) -- (\offsetX,\offsetX+\offsetY+\transferx ,\latentz) --cycle;
    
    }
  }
\filldraw[red] (3.75,3.75,7) circle (1.5pt);
\draw (4.25,4.25,7) node {$\theta(t)$};
\filldraw[red] (3.75,3.75+10,7) circle (1.5pt);
\draw (4.05,10+4.35,7) node {$\phi(t)$};
\filldraw[cyan] (1,2,3) circle (1.5pt);
\draw (1,3.25,3) node {$F(\theta(t))$};
\filldraw[cyan] (2,13.5,3) circle (1.5pt);
\draw (1.5,10+2.5,3) node {$G(\phi(t))$};
    \draw (5,8.25,5.5) node {$L(F,G)$};
    \draw (1,1,7) node {$\theta$-space};
    \draw (1,11,7) node {$\phi$-space};
    \draw (6,1.5,3) node {$F(\theta)$-space};
    \draw (6,13.5,3) node {$G(\phi)$-space};
    \draw (3,2.5,7)
    node { \scriptsize $ \dot{\theta}_i =-\nabla_{\theta_i}L( F(\theta), G(\phi))$ };
    \draw  (3,12.5,7)
    node { \scriptsize $ \dot{\phi}_j =\nabla_{\phi_j}L( F(\theta), G(\phi))$ };
    \def\transfery{0.25}
    \filldraw[thick,-,cyan,opacity=0.7] (4,4+5+\transfery,6.5) --(5,4+5+\transfery,6.5)--(5,4+5+\transfery,4.5)--(4,4+5+\transfery,4.5);
    \filldraw[thick,-,cyan,opacity=0.7]  (4,4+3+\transfery,6.5) -- (5,4+3+\transfery,6.5)--(5,4+5+\transfery,6.5)--(4,4+5+\transfery,6.5)--cycle;
    \filldraw[thick,-,cyan,opacity=0.4] (5,4+3+\transfery,4.5)--(5,4+5+\transfery,4.5)--(5,4+5+\transfery,6.5) -- (5,4+3+\transfery,6.5)--cycle;

    \def\transfery{0.25}
    \filldraw[thick,-,cyan] (5,2.5,5.5) circle (15pt);
    \draw (5,2.5,5.5) node {$F$};
    \filldraw[thick,-,cyan] (5,14,5.5) circle (15pt);
    \draw (5,14,5.5) node {$G$};
    
    
\end{tikzpicture}


==> figures/safety.tex <==

\begin{tikzpicture}
  \draw[->] (-5, 0) -- (6, 0) node[right] {$\mathbf{\theta}$};
  \draw[->] (0, -0.5) -- (0, 5) node[above] {$F(\mathbf{\theta})$};
  \draw[domain=-5:6, samples=1000, variable=\x, blue] plot ({\x}, {3*( (\x+2)^2*exp(-((\x+2)^4/4)) +  
  (\x)^2*exp(-((\x)^2/2)) - ((\x-2)/8)^2*exp(-((\x-2)^2/4)) )
  });
  
  \def\A{-3.15};
  \def\B{-2.27};
  \def\C{-0.96};
  \def\D{0.122};
  \def\E{1.42};
  \def\F{4.316};
  
  \draw[thick,domain=-5:\A, samples=1000, variable=\x, violet] plot ({\x}, {3*( (\x+2)^2*exp(-((\x+2)^4/4)) +  
  (\x)^2*exp(-((\x)^2/2)) - ((\x-2)/8)^2*exp(-((\x-2)^2/4)) )
  });
  \draw[thick,domain=\A:\B, samples=1000, variable=\x, gray] plot ({\x}, {3*( (\x+2)^2*exp(-((\x+2)^4/4)) +  
  (\x)^2*exp(-((\x)^2/2)) - ((\x-2)/8)^2*exp(-((\x-2)^2/4)) )
  });
  \draw[thick,domain=\B:\C, samples=1000, variable=\x, cyan] plot ({\x}, {3*( (\x+2)^2*exp(-((\x+2)^4/4)) +  
  (\x)^2*exp(-((\x)^2/2)) - ((\x-2)/8)^2*exp(-((\x-2)^2/4)) )
  });
  \draw[thick,domain=\C:\D, samples=1000, variable=\x, brown] plot ({\x}, {3*( (\x+2)^2*exp(-((\x+2)^4/4)) +  
  (\x)^2*exp(-((\x)^2/2)) - ((\x-2)/8)^2*exp(-((\x-2)^2/4)) )
  });
  \draw[thick,domain=\D:\E, samples=1000, variable=\x, magenta] plot ({\x}, {3*( (\x+2)^2*exp(-((\x+2)^4/4)) +  
  (\x)^2*exp(-((\x)^2/2)) - ((\x-2)/8)^2*exp(-((\x-2)^2/4)) )
  });
  \draw[thick,domain=\E:\F, samples=1000, variable=\x, orange] plot ({\x}, {3*( (\x+2)^2*exp(-((\x+2)^4/4)) +  
  (\x)^2*exp(-((\x)^2/2)) - ((\x-2)/8)^2*exp(-((\x-2)^2/4)) )
  });
  \draw[thick,domain=\F:6, samples=1000, variable=\x, blue] plot ({\x}, {3*( (\x+2)^2*exp(-((\x+2)^4/4)) +  
  (\x)^2*exp(-((\x)^2/2)) - ((\x-2)/8)^2*exp(-((\x-2)^2/4)) )
  });
  \foreach\m in {\A,\B,\C,\D,\E,\F}
  {
    \def\k{\m-0.65}
    \filldraw[red] (\k,{3*( (\k+2)^2*exp(-((\k+2)^4/4)) +   (\k)^2*exp(-((\k)^2/2)) -   ((\k-2)/8)^2*exp(-((\k-2)^2/4)) )}) circle (1pt);
    \def\fm{3*( (\m+2)^2*exp(-((\m+2)^4/4)) +    (\m)^2*exp(-((\m)^2/2)) - ((\m-2)/8)^2*exp(-((\m-2)^2/4)) )};
    \draw[-] (\m, {\fm-0.2}) -- (\m, {\fm+0.2});
  }
\end{tikzpicture}

